Every Annotation Counts: Multi-label Deep Supervision for Medical Image Segmentation

Pixel-wise segmentation is one of the most data and annotation hungry tasks in our field. Providing representative and accurate annotations is often mission-critical especially for challenging medical applications. In this paper, we propose a semi-weakly supervised segmentation algorithm to overcome this barrier. Our approach is based on a new formulation of deep supervision and student-teacher model and allows for easy integration of different supervision signals. In contrast to previous work, we show that care has to be taken how deep supervision is integrated in lower layers and we present multi-label deep supervision as the most important secret ingredient for success. With our novel training regime for segmentation that flexibly makes use of images that are either fully labeled, marked with bounding boxes, just global labels, or not at all, we are able to cut the requirement for expensive labels by 94.22% - narrowing the gap to the best fully supervised baseline to only 5% mean IoU. Our approach is validated by extensive experiments on retinal fluid segmentation and we provide an in-depth analysis of the anticipated effect each annotation type can have in boosting segmentation performance.

==> latex/figures/evaluation_figures/eval_figure2.tex <==
% \begin{figure*}[t]
%   \includegraphics[width=\textwidth,height=0.25\textwidth]{example-image-a}
%   \caption{THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE RESULTS GO. THIS IS WHERE QUALITATIVE.}
%   \label{fig:method}
% \end{figure*}

==> latex/figures/method_figure_all/method_figure3.tex <==
\begin{figure}[t]
  \centering
  \includegraphics[height=0.8\linewidth]{latex/figures/method_figure_all/pseudo-label-deep-supervision_crop.pdf}
  \caption{Smoothing effect of deep multi-label supervision on pseudo-labels: By down-sampling pseudo-labels, at smaller scales, their erroneous predictions like small shifts or few missed pixel-classifications get smoothed out and match the ground-truth.}
  \label{fig:pseudo-label-smoothing}
\end{figure}

==> latex/tables/bounding_box_results.tex <==
\setlength{\tabcolsep}{4.5pt}

\begin{table*}[t]
\centering
\begin{tabular}{r|cc|c|c|c|c||c|}
    Method & $\mathcal{G}$ & $\mathcal{U}$ & $\mathcal{B}(3)$ & $\mathcal{B}(6)$ & $\mathcal{B}(12)$ & $\mathcal{B}(24)$ & $\mathcal{B}(\textbf{full})$\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $12.49 \pm 4.28$ & $18.32 \pm 4.94$ & $25.62 \pm 3.08$ & $29.55 \pm 2.77$ & $38.45 \pm 4.44$\\
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $\underline{15.40} \pm \underline{7.07}$ & $18.15 \pm 7.49$ & $26.05 \pm 6.00$ & $30.07 \pm 4.32$ & $38.45 \pm 4.65$\\
    MIL Baseline & \checkmark &  & $15.82 \pm 6.55$ & $16.95 \pm 6.19$ & $22.56 \pm 4.56$ & $26.48 \pm 5.51$ & $37.15 \pm 4.06$\\
    \cdashline{1-8}
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $12.77 \pm 7.15$ & $17.76 \pm 6.26$ & $\underline{28.99} \pm \underline{4.60}$ & $30.64 \pm 3.05$ & $38.81 \pm 4.48$\\
    Deeply Supervised MIL & \checkmark &  & $\textbf{17.14} \pm \textbf{8.06}$ & $20.18 \pm 4.61$ & $24.15 \pm 4.95$ & $29.12 \pm 4.75$ & $37.94 \pm 3.35$\\
    \cdashline{1-8}
    Perone et al.$^{10}$~\cite{perone2018deep} &  & \checkmark & $11.17 \pm 7.41$ & $19.02 \pm 8.46$ & $27.44 \pm 5.81$ & $31.72 \pm 3.87$ & $39.38 \pm 3.56$\\
    \cdashline{1-8}
    Multi-Label Deep Supervision &  &  & $14.59 \pm 5.81$ & $\underline{19.62} \pm \underline{6.21}$ & $27.89 \pm 3.44$ & $32.02 \pm 4.78$ & $38.66 \pm 3.36$\\
    Self-Taught Deep Supervision &  & \checkmark & $5.14 \pm 3.84$ & $9.62 \pm 7.35$ & $24.47 \pm 6.12$ & $32.71 \pm 3.56$ & $\underline{\textbf{39.39}} \pm \underline{\textbf{3.63}}$\\
    Self-Taught Deep Supervision & \checkmark &  & $16.04 \pm 8.52$ & $\textbf{22.15} \pm \textbf{6.29}$ & $28.63 \pm 4.04$ & $32.37 \pm 3.75$ & $38.97 \pm 3.59$\\
    Mean-Taught Deep Supervision$^{10}$ &  & \checkmark & $8.21 \pm 3.96$ & $14.28 \pm 7.48$ & $24.79 \pm 5.79$ & $\underline{34.14} \pm \underline{3.10}$ & $39.04 \pm 4.15$\\
    Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & $15.81 \pm 8.59$ & $21.97 \pm 8.17$ & $\textbf{29.83} \pm \textbf{5.30}$ & $\textbf{34.81} \pm \textbf{3.62}$ & $38.66 \pm 4.73$\\
    \hline
\end{tabular}
\caption{Bounding box supervision. Testing performance (\underline{best semi-supervised}, \textbf{best semi-weakly supervised}). Superscript in method names indicate a different batch size than 16.}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{r|cc|c|c|c|c||c|}
%     Method & $\mathcal{G}$ & $\mathcal{U}$ & $\mathcal{B}(3)$ & $\mathcal{B}(6)$ & $\mathcal{B}(12)$ & $\mathcal{B}(24)$ & $\mathcal{B}(\textbf{full})$\\
%     \hline
%     Baseline~\cite{ronneberger2015u} &  &  & $11.02 \pm 4.73$ & $16.83 \pm 6.46$ & $22.72 \pm 7.87$ & $30.59 \pm 5.40$ & $39.65 \pm 3.12$\\
%     IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $13.86 \pm 7.53$ & $19.19 \pm 9.64$ & $25.39 \pm 6.99$ & $32.70 \pm 7.44$ & $40.78 \pm 2.82$\\
%     MIL Baseline & \checkmark &  & $17.71 \pm 7.58$ & $19.41 \pm 6.74$ & $26.58 \pm 5.38$ & $27.73 \pm 7.53$ & $39.02 \pm 3.71$\\
%     \cdashline{1-8}
%     Deeply Supervised IIC$^{8}$ &  & \checkmark & $12.35 \pm 6.67$ & $17.78 \pm 7.96$ & $27.23 \pm 8.44$ & $33.32 \pm 7.58$ & $39.26 \pm 2.31$\\
%     Deeply Supervised MIL & \checkmark &  &$17.95 \pm 7.17$ & $24.19 \pm 2.88$ & $25.42 \pm 5.87$ & $31.07 \pm 5.25$ & $38.98 \pm 3.00$\\
%     \cdashline{1-8}
%     Perone et al.$^{10}$~\cite{perone2018deep} &  & \checkmark & $12.95 \pm 6.97$ & $18.06 \pm 8.67$ & $26.72 \pm 7.05$ & $34.76 \pm 4.55$ & $40.24 \pm 2.38$\\
%     \cdashline{1-8}
%     Multi-Label Deep Supervision &  &  & $13.29 \pm 5.17$ & $17.59 \pm 5.79$ & $27.47 \pm 7.61$ & $32.88 \pm 6.87$ & $39.64 \pm 2.47$\\
%     Self-Taught Deep Supervision &  & \checkmark & $5.59 \pm 4.02$ & $9.86 \pm 6.42$ & $22.88 \pm 7.67$ & $31.75 \pm 6.67$ & $39.64 \pm 3.18$\\
%     Self-Taught Deep Supervision & \checkmark &  & $14.66 \pm 5.37$ & $20.54 \pm 6.52$ & $26.29 \pm 7.74$ & $32.02 \pm 5.77$ & $40.59 \pm 3.50$\\
%     Mean-Taught Deep Supervision$^{10}$ &  & \checkmark & $7.64 \pm 2.15$ & $14.62 \pm 5.47$ & $24.65 \pm 7.87$ & $37.34 \pm 4.77$ & $39.97 \pm 2.08$\\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & $15.20 \pm 6.08$ & $22.42 \pm 7.55$ & $31.67 \pm 6.43$ & $37.38 \pm 5.38$ & $40.01 \pm 2.29$\\
%     \hline
% \end{tabular}
% \caption{Validation performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}

==> latex/tables/mask_results.tex <==
\setlength{\tabcolsep}{4.5pt}

\begin{table*}[t]
\centering
\begin{tabular}{r|cc|c|c|c|c||c|}
    Method & $\mathcal{G}$ & $\mathcal{U}$ & $\mathcal{M}(3)$ & $\mathcal{M}(6)$ & $\mathcal{M}(12)$ & $\mathcal{M}(24)$ & $\mathcal{M}(\textbf{full})$\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $14.80 \pm 6.50$ & $26.98 \pm 7.83$ & $35.39 \pm 6.36$ & $48.63 \pm 5.17$ & $62.09 \pm 4.77$\\
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $\underline{\textbf{22.45}} \pm \underline{\textbf{9.36}}$ & $32.02 \pm 7.23$ & $41.48 \pm 7.26$ & $53.08 \pm 6.13$ & $65.16 \pm 3.80$\\
    MIL Baseline & \checkmark &  & $15.44 \pm 11.10$ & $25.46 \pm 8.57$ & $41.34 \pm 9.66$ & $49.07 \pm 8.20$ & $61.50 \pm 5.64$\\
    \cdashline{1-8}
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $20.78 \pm 8.83$ & $31.39 \pm 10.26$ & $39.18 \pm 6.94$ & $50.10 \pm 7.92$ & $65.18 \pm 3.85$\\
    Deeply Supervised MIL & \checkmark &  & $20.02 \pm 9.17$ & $31.50 \pm 8.88$ & $44.29 \pm 5.03$ & $51.13 \pm 3.93$ & $62.04 \pm 3.92$\\
    \cdashline{1-8}
    Perone et al.$^{10}$~\cite{perone2018deep} &  & \checkmark & $16.17 \pm 10.74$ & $33.10 \pm 10.24$ & $45.80 \pm 7.51$ & $54.75 \pm 5.96$ & $65.49 \pm 4.14$\\
    \cdashline{1-8}
    Multi-Label Deep Supervision &  &  & $17.98 \pm 8.20$ & $32.92 \pm 7.35$ & $42.96 \pm 6.71$ & $52.68 \pm 6.82$ & $65.82 \pm 4.64$\\
    Self-Taught Deep Supervision &  & \checkmark & $10.37 \pm 8.29$ & $28.62 \pm 12.96$ & $43.57 \pm 9.97$ & $56.11 \pm 6.30$ & $66.24 \pm 4.67$\\
    Self-Taught Deep Supervision & \checkmark &  & $20.47 \pm 8.62$ & $36.40 \pm 8.91$ & $49.39 \pm 9.95$ & $59.29 \pm 7.52$ & $66.34 \pm 3.81$\\
    Mean-Taught Deep Supervision$^{10}$ &  & \checkmark & $16.31 \pm 15.48$ & $\underline{35.17} \pm \underline{11.35}$ & $\underline{53.52} \pm \underline{8.72}$ & $\underline{58.84} \pm \underline{6.57}$ & $\underline{66.31} \pm \underline{4.66}$\\
    Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & $21.91 \pm 13.49$ & $\textbf{42.14} \pm \textbf{14.25}$ & $\textbf{54.70} \pm \textbf{9.26}$   & $\textbf{60.45} \pm \textbf{5.71}$ & $\textbf{66.39} \pm \textbf{4.29}$\\
    \hline
\end{tabular}
\caption{Pixel-wise supervision. Testing performance (\underline{best semi-supervised}, \textbf{best semi-weakly supervised}). Superscript in method names indicate a different batch size than 16.}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}{r|cc|c|c|c|c||c|}
%     Method & $\mathcal{G}$ & $\mathcal{U}$ & $\mathcal{M}(3)$ & $\mathcal{M}(6)$ & $\mathcal{M}(12)$ & $\mathcal{M}(24)$ & $\mathcal{M}(\textbf{full})$\\
%     \hline
%     Baseline~\cite{ronneberger2015u} &  &  & $13.78 \pm 7.38$ & $23.29 \pm 7.84$ & $32.11 \pm 7.00$ & $46.84 \pm 6.49$ & $62.42 \pm 4.11$\\
%     IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $20.06 \pm 7.52$ & $30.47 \pm 10.80$ & $40.87 \pm 10.32$ & $52.82 \pm 7.17$ & $64.33 \pm 2.84$\\
%     MIL Baseline & \checkmark &  & $14.80 \pm 10.39$ & $23.64 \pm 11.86$ & $38.56 \pm 12.42$ & $49.48 \pm 4.88$ & $61.92 \pm 4.77$\\
%     \cdashline{1-8}
%     Deeply Supervised IIC$^{8}$ &  & \checkmark & $20.67 \pm 7.63$ & $28.53 \pm 11.93$ & $42.45 \pm 8.70$ & $53.63 \pm 4.69$ & $65.23 \pm 3.58$\\
%     Deeply Supervised MIL & \checkmark &  & $18.83 \pm 7.98$ & $28.16 \pm 9.71$ & $44.71 \pm 8.25$ & $53.52 \pm 4.69$ & $63.03 \pm 3.10$\\
%     \cdashline{1-8}
%     Perone et al.$^{10}$~\cite{perone2018deep} &  & \checkmark & $14.79 \pm 8.15$ & $31.77 \pm 10.43$ & $46.52 \pm 7.68$ & $56.51 \pm 5.56$ & $64.77 \pm 2.90$\\
%     \cdashline{1-8}
%     Multi-Label Deep Supervision &  &  & $14.89 \pm 8.16$ & $29.02 \pm 9.91$ & $39.63 \pm 7.74$ & $52.03 \pm 5.48$ & $65.45 \pm 2.89$\\
%     Self-Taught Deep Supervision &  & \checkmark & $9.28 \pm 4.09$ & $28.13 \pm 13.26$ & $43.86 \pm 12.44$ & $54.13 \pm 7.38$ & $64.97 \pm 2.96$\\
%     Self-Taught Deep Supervision & \checkmark &  & $17.64 \pm 8.20$ & $34.57 \pm 12.99$ & $48.36 \pm 9.54$ & $57.80 \pm 4.68$ & $64.97 \pm 2.48$\\
%     Mean-Taught Deep Supervision$^{10}$ &  & \checkmark & $14.86 \pm 13.35$ & $34.22 \pm 9.17$ & $52.02 \pm 7.01$ & $60.63 \pm 5.35$ & $66.54 \pm 3.15$\\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & $17.41 \pm 10.70$ & $38.31 \pm 11.32$ & $55.86 \pm 4.89$ & $61.36 \pm 4.73$ & $66.32 \pm 3.71$\\
%     \hline
% \end{tabular}
% \caption{Validation performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}


==> latex/tables/merged_mask_bb.tex <==
\setlength{\tabcolsep}{2.5pt}

\begin{table*}[t]
\centering
\begin{tabular}{r|cc|c|c|c|c||c|}
    Method & $\mathcal{G}$ & $\mathcal{U}$ & $3$ & $6$ & $12$ & $24$ & Full Access \\
    \hline
    &&&\multicolumn{5}{c|}{\textbf{Mask Supervision}}\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $14.80 \pm 6.50$ & $26.98 \pm 7.83$ & $35.39 \pm 6.36$ & $48.63 \pm 5.17$ & $62.09 \pm 4.77$\\
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $\underline{\textbf{22.45}} \pm \underline{\textbf{9.36}}$ & $32.02 \pm 7.23$ & $41.48 \pm 7.26$ & $53.08 \pm 6.13$ & $65.16 \pm 3.80$\\
    MIL Baseline & \checkmark &  & $15.44 \pm 11.10$ & $25.46 \pm 8.57$ & $41.34 \pm 9.66$ & $49.07 \pm 8.20$ & $61.50 \pm 5.64$\\
    \cdashline{1-8}
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $20.78 \pm 8.83$ & $31.39 \pm 10.26$ & $39.18 \pm 6.94$ & $50.10 \pm 7.92$ & $65.18 \pm 3.85$\\
    Deeply Supervised MIL & \checkmark &  & $20.02 \pm 9.17$ & $31.50 \pm 8.88$ & $44.29 \pm 5.03$ & $51.13 \pm 3.93$ & $62.04 \pm 3.92$\\
    \cdashline{1-8}
    \emph{Perone and Cohen-Adad}$^{10}$~\cite{perone2018deep} &  & \checkmark & $16.17 \pm 10.74$ & $33.10 \pm 10.24$ & $45.80 \pm 7.51$ & $54.75 \pm 5.96$ & $65.49 \pm 4.14$\\
    \cdashline{1-8}
    Multi-Label Deep Supervision (Ours) &  &  & $17.98 \pm 8.20$ & $32.92 \pm 7.35$ & $42.96 \pm 6.71$ & $52.68 \pm 6.82$ & $65.82 \pm 4.64$\\
    Self-Taught Deep Supervision (Ours) &  & \checkmark & $10.37 \pm 8.29$ & $28.62 \pm 12.96$ & $43.57 \pm 9.97$ & $56.11 \pm 6.30$ & $66.24 \pm 4.67$\\
    Self-Taught Deep Supervision (Ours) & \checkmark &  & $20.47 \pm 8.62$ & $36.40 \pm 8.91$ & $49.39 \pm 9.95$ & $59.29 \pm 7.52$ & $66.34 \pm 3.81$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) &  & \checkmark & $16.31 \pm 15.48$ & $\underline{35.17} \pm \underline{11.35}$ & $\underline{53.52} \pm \underline{8.72}$ & $\underline{58.84} \pm \underline{6.57}$ & $\underline{66.31} \pm \underline{4.66}$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) & \checkmark &  & $21.91 \pm 13.49$ & $\textbf{42.14} \pm \textbf{14.25}$ & $\textbf{54.70} \pm \textbf{9.26}$   & $\textbf{60.45} \pm \textbf{5.71}$ & $\textbf{66.39} \pm \textbf{4.29}$\\
    \hline
    &&&\multicolumn{5}{c|}{\textbf{Bounding Box Supervision}}\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $12.49 \pm 4.28$ & $18.32 \pm 4.94$ & $25.62 \pm 3.08$ & $29.55 \pm 2.77$ & $38.45 \pm 4.44$\\
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $\underline{15.40} \pm \underline{7.07}$ & $18.15 \pm 7.49$ & $26.05 \pm 6.00$ & $30.07 \pm 4.32$ & $38.45 \pm 4.65$\\
    MIL Baseline & \checkmark &  & $15.82 \pm 6.55$ & $16.95 \pm 6.19$ & $22.56 \pm 4.56$ & $26.48 \pm 5.51$ & $37.15 \pm 4.06$\\
    \cdashline{1-8}
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $12.77 \pm 7.15$ & $17.76 \pm 6.26$ & $\underline{28.99} \pm \underline{4.60}$ & $30.64 \pm 3.05$ & $38.81 \pm 4.48$\\
    Deeply Supervised MIL & \checkmark &  & $\textbf{17.14} \pm \textbf{8.06}$ & $20.18 \pm 4.61$ & $24.15 \pm 4.95$ & $29.12 \pm 4.75$ & $37.94 \pm 3.35$\\
    \cdashline{1-8}
    \emph{Perone and Cohen-Adad}$^{10}$~\cite{perone2018deep} &  & \checkmark & $11.17 \pm 7.41$ & $19.02 \pm 8.46$ & $27.44 \pm 5.81$ & $31.72 \pm 3.87$ & $39.38 \pm 3.56$\\
    \cdashline{1-8}
    Multi-Label Deep Supervision (Ours) &  &  & $14.59 \pm 5.81$ & $\underline{19.62} \pm \underline{6.21}$ & $27.89 \pm 3.44$ & $32.02 \pm 4.78$ & $38.66 \pm 3.36$\\
    Self-Taught Deep Supervision (Ours) &  & \checkmark & $5.14 \pm 3.84$ & $9.62 \pm 7.35$ & $24.47 \pm 6.12$ & $32.71 \pm 3.56$ & $\underline{\textbf{39.39}} \pm \underline{\textbf{3.63}}$\\
    Self-Taught Deep Supervision (Ours) & \checkmark &  & $16.04 \pm 8.52$ & $\textbf{22.15} \pm \textbf{6.29}$ & $28.63 \pm 4.04$ & $32.37 \pm 3.75$ & $38.97 \pm 3.59$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) &  & \checkmark & $8.21 \pm 3.96$ & $14.28 \pm 7.48$ & $24.79 \pm 5.79$ & $\underline{34.14} \pm \underline{3.10}$ & $39.04 \pm 4.15$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) & \checkmark &  & $15.81 \pm 8.59$ & $21.97 \pm 8.17$ & $\textbf{29.83} \pm \textbf{5.30}$ & $\textbf{34.81} \pm \textbf{3.62}$ & $38.66 \pm 4.73$\\
    \hline
\end{tabular}
\caption{Results for a diverse variety of models using varying amounts ($3$,$6$,$12$,$24$,all) of annotations, i.e. ground-truth masks or coarse bounding boxes. Performance in average mIoU over 10 testing splits with standard deviation (\underline{best semi-supervised}, \textbf{best semi-weakly supervised}). $\mathcal{U}$ uses additional unlabeled images, $\mathcal{G}$ global image labels. Superscripts indicate smaller batch sizes due to memory constraints.}
\label{tab:mask_and_boundingbox}
\end{table*}



==> latex/tables/supp_iic_clusters.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|c|c|c|c}
    $\#\text{epochs}$& $\mathcal{U}$ & \#clusters & $f$ & validation (mIoU)\\
    \hline
    $100$ & & -- & -- & $62.42 \pm 4.11$ \\
    $200$ & & -- & -- & $62.54 \pm 3.88$ \\
    \cdashline{1-5}
    $100$ & \checkmark & $5$ & $f_4$ & $63.42 \pm 4.32$ \\
    $100$ & \checkmark & $10$ & $f_4$ & $64.33 \pm 2.84$ \\
    $100$ & \checkmark & $20$ & $f_4$ & $64.63 \pm 3.36$ \\
    \cdashline{1-5}
    $100$* & \checkmark & 10 & $f_{\{0-4\}}$ & $\textbf{65.23} \pm \textbf{3.58}$ \\
    % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1,2,3 & $-- \pm --$ & $-- \pm --$ \\
    % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1,2 & $-- \pm --$ & $-- \pm --$ \\
    % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1 & $-- \pm --$ & $-- \pm --$ \\
    % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0 & $-- \pm --$ & $-- \pm --$ \\
    \hline
\end{tabular}
\caption{Ablation for the number of heads for IIC models. Due to high memory consumption, we reduce the batch size from 16 to 8 for the model with the * symbol. All models are trained with full access to pixel-wise annotated masks.}
\label{tab:iic_heads}
\end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{r|l|c|c|l|l|l|l}
%     & Supervision & \#clusters& hierarchies & mIoU val & mIoU test \\
%     \hline
%     UNet (100 epochs) & $\mathcal{M}$ (\textbf{all}) & -- & -- & $62.42 \pm 4.11$ & $62.09 \pm 4.77$\\
%     UNet (200 epochs) & $\mathcal{M}$ (\textbf{all}) & -- & -- & $62.54 \pm 3.88$ & $63.77 \pm 4.71$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 5 & 4 & $63.42 \pm 4.32$ & $64.95 \pm 4.78$ \\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 4 & $64.33 \pm 2.84$ & $65.16 \pm 3.80$ \\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 20 & 4 & $64.63 \pm 3.36$ & $64.49 \pm 3.31$ \\
%     \hdashline
%     Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1,2,3,4 & $\textbf{65.23} \pm \textbf{3.58}$ & $\textbf{65.18} \pm \textbf{3.85}$ \\
%     % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1,2,3 & $-- \pm --$ & $-- \pm --$ \\
%     % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1,2 & $-- \pm --$ & $-- \pm --$ \\
%     % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0,1 & $-- \pm --$ & $-- \pm --$ \\
%     % Multi-Task UNet* & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & 0 & $-- \pm --$ & $-- \pm --$ \\
%     \hline
% \end{tabular}
% \caption{Ablation for the number of heads for iic loss. Due to high memory constraints, we reduce the batchsize from 16 to 8, models trained with reduced batch size are listed with the *-symbol.}
% \label{tab:iic_heads}
% \end{table}

==> latex/tables/supp_mil_hierarchies.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|c|c}
    $\mathcal{G}$& $f$ & validation (mIoU) \\
    \hline
    & -- & $46.84 \pm 6.49$ \\
    \cdashline{1-3}
    \checkmark & $f_4$ & $49.48 \pm 4.88$ \\
    \checkmark & $f_{\{3,4\}}$ & $50.13 \pm 6.25$ \\
    \checkmark & $f_{\{2,3,4\}}$ & $51.81 \pm 5.58$ \\
    \checkmark & $f_{\{1,2,3,4\}}$ & $51.47 \pm 4.03$\\
    \checkmark & $f_{\{0,1,2,3,4\}}$ & $\textbf{53.52} \pm \textbf{4.69}$ \\
    \checkmark & $f_{\{0,1,2,3\}}$ & $52.85 \pm 4.50$ \\
    \checkmark & $f_{\{0,1,2\}}$ & $51.81 \pm 6.25$ \\
    \checkmark & $f_{\{0,1\}}$ & $51.68 \pm 5.48$ \\
    \checkmark & $f_0$ & $50.23 \pm 7.38$ \\
    \hline
\end{tabular}
\caption{Ablation for enforcing the image-level MIL loss on different feature maps within the UNet. First line indicates performance without image-level labels, second line indicates what we refer to in the paper as \emph{Baseline MIL}, the best performing model here is the \emph{Deeply Supervised MIL} model in the paper.}
\label{tab:image-level_hierarchies}
\end{table}


% \begin{table}[]
% \centering
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & hierarchies & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (24) & -- & $46.84 \pm 6.49$& $48.63 \pm 5.17$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 4 & $49.48 \pm 4.88$ & $49.07 \pm 8.20$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 3,4 & $50.13 \pm 6.25$ & $48.73 \pm 6.28$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 2,3,4 & $51.81 \pm 5.58$ & $49.89 \pm 7.29$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 1,2,3,4 & $51.47 \pm 4.03$ & $51.31 \pm 5.03$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 0,1,2,3,4 & $\textbf{53.52} \pm \textbf{4.69}$ & $51.13 \pm 3.93$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 0,1,2,3 & $52.85 \pm 4.50$ & $51.15 \pm 6.06$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 0,1,2 & $51.81 \pm 6.25$ & $50.65 \pm 6.20$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 0,1 & $51.68 \pm 5.48$ & $\textbf{52.41} \pm \textbf{7.18}$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 0 & $50.23 \pm 7.38$ & $50.44 \pm 7.62$ \\
%     \hline
% \end{tabular}
% \caption{Ablation for enforcing the loss image-level MIL loss on varying hierarchies within the UNet architecture.}
% \label{tab:image-level_hierarchies}
% \end{table}

==> latex/tables/supp_milpooling.tex <==
\begin{table}[]
\centering
\begin{tabular}{c|c|c}
    $\mathcal{G}$ & pooling function & validation (mIoU) \\
    \hline
    & -- & $46.84 \pm 6.49$ \\
    \cdashline{1-3}
    \checkmark & max pooling & $46.96 \pm 12.73$ \\
    \checkmark & average pooling & $\textbf{53.52} \pm \textbf{4.69}$ \\
    \hline
\end{tabular}
\caption{Ablation of pooling functions for MIL-based models with access to $24$ pixel-wise masks and global labels are provided.}
\label{tab:mil_pooling}
\end{table}

% \begin{table}[]
% \centering
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & pooling function & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (24) & -- & $46.84 \pm 6.49$& $48.63 \pm 5.17$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & max pooling & $46.96 \pm 12.73$ & $47.79 \pm 4.78$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & average pooling & $\textbf{53.52} \pm \textbf{4.69}$ & $\textbf{51.13} \pm \textbf{3.93}$ \\
%     \hline
% \end{tabular}
% \caption{Ablation for the pooling function for the image-level MIL loss.}
% \label{tab:mil_pooling}
% \end{table}

==> latex/tables/supp_validation_results.tex <==
\setlength{\tabcolsep}{2.5pt}
\begin{table*}[t]
\centering
\begin{tabular}{r|cc|c|c|c|c||c|}
    Method & $\mathcal{G}$ & $\mathcal{U}$ & $3$ & $6$ & $12$ & $24$ & Full Access \\
    \hline
    &&&\multicolumn{5}{c|}{\textbf{Mask Supervision}}\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $13.78 \pm \phantom{0}7.38$ & $23.29 \pm \phantom{0}7.84$ & $32.11 \pm \phantom{0}7.00$ & $46.84 \pm \phantom{0}6.49$ & $62.42 \pm \phantom{0}4.11$ \\
    Multi-Label Deep Supervision (Ours) &  &  & $\textbf{14.89} \pm \phantom{0}\textbf{8.16}$ & $\textbf{29.02} \pm \phantom{0}\textbf{9.91}$ & $\textbf{39.63} \pm \phantom{0}\textbf{7.74}$ & $\textbf{52.03} \pm \phantom{0}\textbf{5.48}$ & $\textbf{65.45} \pm \phantom{0}\textbf{2.89}$\\
    \cdashline{1-8}
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $20.06 \pm \phantom{0}7.52$ & $30.47 \pm 10.80$ & $40.87 \pm 10.32$ & $52.82 \pm \phantom{0}7.17$ & $64.33 \pm \phantom{0}2.84$\\
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $\textbf{20.67} \pm \phantom{0}\textbf{7.63}$ & $28.53 \pm 11.93$ & $42.45 \pm \phantom{0}8.70$ & $53.63 \pm \phantom{0}4.69$ & $65.23 \pm \phantom{0}3.58$\\
    \emph{Perone and Cohen-Adad}$^{10}$~\cite{perone2018deep} &  & \checkmark & $14.79 \pm \phantom{0}8.15$ & $31.77 \pm 10.43$ & $46.52 \pm \phantom{0}7.68$ & $56.51 \pm \phantom{0}5.56$ & $64.77 \pm \phantom{0}2.90$\\
    Self-Taught Deep Supervision (Ours) &  & \checkmark & $9.28 \pm \phantom{0}4.09$ & $28.13 \pm 13.26$ & $43.86 \pm 12.44$ & $54.13 \pm \phantom{0}7.38$ & $64.97 \pm \phantom{0}2.96$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) &  & \checkmark & $14.86 \pm 13.35$ & $\textbf{34.22} \pm \phantom{0}\textbf{9.17}$ & $\textbf{52.02} \pm \phantom{0}\textbf{7.01}$ & $\textbf{60.63} \pm \phantom{0}\textbf{5.35}$ & $\textbf{66.54} \pm \phantom{0}\textbf{3.15}$\\
    \cdashline{1-8}
    MIL Baseline & \checkmark &  & $14.80 \pm 10.39$ & $23.64 \pm 11.86$ & $38.56 \pm 12.42$ & $49.48 \pm \phantom{0}4.88$ & $61.92 \pm \phantom{0}4.77$\\
    Deeply Supervised MIL & \checkmark &  & $\textbf{18.83} \pm \phantom{0}\textbf{7.98}$ & $28.16 \pm \phantom{0}9.71$ & $44.71 \pm \phantom{0}8.25$ & $53.52 \pm \phantom{0}4.69$ & $63.03 \pm \phantom{0}3.10$\\
    Self-Taught Deep Supervision (Ours) & \checkmark &  & $17.64 \pm \phantom{0}8.20$ & $34.57 \pm 12.99$ & $48.36 \pm \phantom{0}9.54$ & $57.80 \pm \phantom{0}4.68$ & $64.97 \pm \phantom{0}2.48$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) & \checkmark &  & $17.41 \pm 10.70$ & $\textbf{38.31} \pm \textbf{11.32}$ & $\textbf{55.86} \pm \phantom{0}\textbf{4.89}$ & $\textbf{61.36} \pm \phantom{0}\textbf{4.73}$ & $\textbf{66.32} \pm \phantom{0}\textbf{3.71}$\\
    \hline
    &&&\multicolumn{5}{c|}{\textbf{Bounding Box Supervision}}\\
    \hline
    Baseline~\cite{ronneberger2015u} &  &  & $11.02 \pm 4.73$ & $16.83 \pm 6.46$ & $22.72 \pm 7.87$ & $30.59 \pm 5.40$ & $\textbf{39.65} \pm \textbf{3.12}$\\
    Multi-Label Deep Supervision (Ours) &  &  & $\textbf{13.29} \pm \textbf{5.17}$ & $\textbf{17.59} \pm \textbf{5.79}$ & $\textbf{27.47} \pm \textbf{7.61}$ & $\textbf{32.88} \pm \textbf{6.87}$ & $39.64 \pm 2.47$\\
    \cdashline{1-8}
    IIC Baseline$^{8}$~\cite{ji2019invariant} &  & \checkmark & $\textbf{13.86} \pm \textbf{7.53}$ & $\textbf{19.19} \pm \textbf{9.64}$ & $25.39 \pm 6.99$ & $32.70 \pm 7.44$ & $\textbf{40.78} \pm \textbf{2.82}$\\
    Deeply Supervised IIC$^{8}$ &  & \checkmark & $12.35 \pm 6.67$ & $17.78 \pm 7.96$ & $\textbf{27.23} \pm \textbf{8.44}$ & $33.32 \pm 7.58$ & $39.26 \pm 2.31$\\
    \emph{Perone and Cohen-Adad}$^{10}$~\cite{perone2018deep} &  & \checkmark & $12.95 \pm 6.97$ & $18.06 \pm 8.67$ & $26.72 \pm 7.05$ & $34.76 \pm 4.55$ & $40.24 \pm 2.38$\\
    Self-Taught Deep Supervision (Ours) &  & \checkmark & $5.59 \pm 4.02$ & $9.86 \pm 6.42$ & $22.88 \pm 7.67$ & $31.75 \pm 6.67$ & $39.64 \pm 3.18$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) &  & \checkmark & $7.64 \pm 2.15$ & $14.62 \pm 5.47$ & $24.65 \pm 7.87$ & $\textbf{37.34} \pm \textbf{4.77}$ & $39.97 \pm 2.08$\\
    \cdashline{1-8}
    MIL Baseline & \checkmark &  & $17.71 \pm 7.58$ & $19.41 \pm 6.74$ & $26.58 \pm 5.38$ & $27.73 \pm 7.53$ & $39.02 \pm 3.71$\\
    Deeply Supervised MIL & \checkmark &  & $\textbf{17.95} \pm \textbf{7.17}$ & $\textbf{24.19} \pm \textbf{2.88}$ & $25.42 \pm 5.87$ & $31.07 \pm 5.25$ & $38.98 \pm 3.00$\\
    Self-Taught Deep Supervision (Ours) & \checkmark &  & $14.66 \pm 5.37$ & $20.54 \pm 6.52$ & $26.29 \pm 7.74$ & $32.02 \pm 5.77$ & $\textbf{40.59} \pm \textbf{3.50}$\\
    Mean-Taught Deep Supervision$^{10}$ (Ours) & \checkmark &  & $15.20 \pm 6.08$ & $22.42 \pm 7.55$ & $\textbf{31.67} \pm \textbf{6.43}$ & $\textbf{37.38} \pm \textbf{5.38}$ & $40.01 \pm 2.29$\\
    \hline
\end{tabular}
\caption{Validation results for a diverse variety of models using varying amounts ($3$,$6$,$12$,$24$,all) of annotations, i.e. ground-truth masks or coarse bounding boxes. Approaches with $\mathcal{U}$ use additional unlabeled images, with $\mathcal{G}$ global image labels (\textbf{best results in category bold}). Performance in average mIoU over 10 testing splits with standard deviation. Superscripts indicate smaller batch sizes due to memory constraints.}
\label{tab:mask_and_boundingbox}
\end{table*}


==> latex/tables/various_experimental_results.tex <==


% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|c|c|c|c|c|c|c|c|}
%     Method & $\mathcal{M} + \mathcal{B}$ & $\mathcal{I}$ & $\mathcal{U}$ & $\mathcal{M}(3)+\mathcal{B}(3)$ &  $\mathcal{M}(6)+\mathcal{B}(6)$ & $\mathcal{M}(12)+\mathcal{B}(12)$\\
%     \hline
%     Baseline & \checkmark &  &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     IIC Baseline & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     MIL Baseline & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     \hdashline
%     Deeply Supervised IIC$^{8}$ & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Deeply Supervised MIL & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     \hdashline
%     Multi-Label Deep Supervision & \checkmark &  &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Self-Taught Deep Supervision & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Self-Taught Deep Supervision & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & \checkmark & $-- \pm --$ & $35.03 \pm 12.34$ & $51.81 \pm 8.07$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark & \checkmark &  & $-- \pm --$ & $42.85 \pm 15.11$ & $54.53 \pm 7.25$ \\
%     \hline
% \end{tabular}
% \caption{Testing performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|c|c|c|c|c|c|c|c|}
%     Method & $\mathcal{M} + \mathcal{B}$ & $\mathcal{I}$ & $\mathcal{U}$ & $\mathcal{M}(3)+\mathcal{B}(3)$ &  $\mathcal{M}(6)+\mathcal{B}(6)$ & $\mathcal{M}(12)+\mathcal{B}(12)$\\
%     \hline
%     Baseline & \checkmark &  &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     IIC Baseline & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     MIL Baseline & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     \hdashline
%     Deeply Supervised IIC$^{8}$ & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Deeply Supervised MIL & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     \hdashline
%     Multi-Label Deep Supervision & \checkmark &  &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Self-Taught Deep Supervision & \checkmark &  & \checkmark & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Self-Taught Deep Supervision & \checkmark & \checkmark &  & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & \checkmark & $-- \pm --$ & $33.40 \pm 12.20$ & $50.93 \pm 7.83$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark & \checkmark &  & $-- \pm --$ & $40.10 \pm 13.99$ & $55.27 \pm 6.15$ \\
%     \hline
% \end{tabular}
% \caption{Validation performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}

% \clearpage















% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|c|c|c|c|c|c|c|c|}
%     Method & $\mathcal{M} + \mathcal{B}$ & $\mathcal{I}$ & $\mathcal{U}$ & $\mathcal{M}(3)+\mathcal{B}(3)$ &  $\mathcal{M}(6)+\mathcal{B}(6)$ & $\mathcal{M}(12)+\mathcal{B}(12)$\\
%     \hline
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & \checkmark & $-- \pm --$ & $27.32 \pm 12.16$ & $43.33 \pm 6.27$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark & \checkmark &  & $-- \pm --$ & $32.45 \pm 13.62$ & $48.60 \pm 8.10$ \\
%     \hdashline
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained & \checkmark &  & \checkmark & $-- \pm --$ & $35.03 \pm 12.34$ & $51.81 \pm 8.07$ \\
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained & \checkmark & \checkmark &  & $-- \pm --$ & $42.85 \pm 15.11$ & $54.53 \pm 7.25$ \\
%     \hdashline
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained (not bkg) & \checkmark &  & \checkmark & $-- \pm --$ & $34.75 \pm 12.74$ & $52.62 \pm 7.10$ \\
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained (not bkg) & \checkmark & \checkmark &  & $-- \pm --$ & $39.84 \pm 13.73$ & $54.79 \pm 9.26$ \\
%     \hline
% \end{tabular}
% \caption{Testing performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}


% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|c|c|c|c|c|c|c|c|}
%     Method & $\mathcal{M} + \mathcal{B}$ & $\mathcal{I}$ & $\mathcal{U}$ & $\mathcal{M}(3)+\mathcal{B}(3)$ &  $\mathcal{M}(6)+\mathcal{B}(6)$ & $\mathcal{M}(12)+\mathcal{B}(12)$\\
%     \hline
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark &  & \checkmark & $-- \pm --$ & $26.87 \pm 11.80$ & $43.50 \pm 7.61$ \\
%     Mean-Taught Deep Supervision$^{10}$ & \checkmark & \checkmark &  & $-- \pm --$ & $31.10 \pm 12.65$ & $48.72 \pm 6.84$ \\
%     \hdashline
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained & \checkmark &  & \checkmark & $-- \pm --$ & $33.40 \pm 12.20$ & $50.93 \pm 7.83$ \\
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained & \checkmark & \checkmark &  & $-- \pm --$ & $40.10 \pm 13.99$ & $55.27 \pm 6.15$ \\
%     \hdashline
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained (not bkg) & \checkmark &  & \checkmark & $-- \pm --$ & $34.15 \pm 10.77$ & $53.76 \pm 6.59$ \\
%     Mean-Taught Deep Supervision$^{10}$ BB-constrained (not bkg) & \checkmark & \checkmark &  & $-- \pm --$ & $37.34 \pm 10.44$ & $55.39 \pm 6.25$ \\
%     \hline
% \end{tabular}
% \caption{Validation performance. Superscript in method names indicate a different batch size than 16.}
% \end{table*}











\clearpage

% \textbf{Output head structure:}

% In Figure~\ref{fig:output_head}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|l|l|l|l|l|l}
%     & Supervision & output head architecture & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (\textbf{all}) & $1 \times 1$ conv. & $62.41 \pm 4.16$ & $63.37 \pm 5.87$ \\
%     UNet & $\mathcal{M}$ (\textbf{all}) & $1 \times 1$ conv. $\to$ BN $\to$ ReLU $\to$ $1 \times 1$ conv.  & $62.42 \pm 4.11$ & $62.09 \pm 4.77$\\
%     \hdashline
%     UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & $1 \times 1$ conv. & $44.42 \pm 5.89$ & $45.06 \pm 4.76$ \\
%     UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & $1 \times 1$ conv. $\to$ BN $\to$ ReLU $\to$ $1 \times 1$ conv.  & $44.07 \pm 7.98$ & $45.48 \pm 6.83$ \\
%     \hline
% \end{tabular}
% \caption{Ablation for the structure of output-heads.}
% \label{fig:output_head}
% \end{table*}

\textbf{Number of clusters for self-supervision:}

In Figure~\ref{fig:iic_heads} we study the performance of a UNet regarding segmentation, when integrating the self-supervised IIC objective on top of the penultimate embeddings.


\textbf{Hierarchical self-supervision integration:}

\textbf{Hierarchical MIL integration:}

We also check how to best integrate image-level signals in an UNet architecture in Figure~\ref{fig:image-level_hierarchies}.



\textbf{MIL pooling function:}




% \textbf{L1-loss:}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & loss function & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (24) & -- & $46.84 \pm 6.49$& $48.63 \pm 5.17$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{U}$ & IIC-loss & $50.74 \pm 7.03$ & $52.04 \pm 6.84$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & average pooling MIL & $53.52 \pm 4.69$ & $51.13 \pm 3.93$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & L1-loss, $\mathcal{I}$-constrained, softmax & $53.50 \pm 5.93$ & $55.18 \pm 5.76$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & L1-loss, $\mathcal{I}$-constrained, sigmoid & $51.90 \pm 7.27$ & $54.74 \pm 6.94$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{U}$ & L1-loss, softmax & $51.47 \pm 7.28$ & $54.48 \pm 4.50$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (24) & BCE binary masks, sigmoid & $51.51 \pm 5.74$ & $52.54 \pm 6.09$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{U}$ & BCE binary masks/predictions, sigmoid & $55.65 \pm 4.75$ & $54.76 \pm 7.35$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & BCE binary masks/predictions, $\mathcal{I}$-constrained, sigmoid & $\textbf{57.24} \pm \textbf{5.74}$ & $57.92 \pm 7.33$ \\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & BCE binary masks/predictions, $\mathcal{I}$-constrained, sigmoid, MIL & $56.86 \pm 3.51$ & $\textbf{58.26} \pm \textbf{6.12}$ \\
%     \hline    
%     \hline
%     UNet & $\mathcal{M}$ (\textbf{all}) & -- & $62.42 \pm 4.11$ & $62.09 \pm 4.77$\\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) & BCE binary masks & $65.39 \pm 3.89$ & $66.66 \pm 3.98$ \\
%     \hline
% \end{tabular}
% \caption{Ablation and comparison for using a L1-loss.}
% \label{fig:output_head}
% \end{table*}



% \begin{table*}[h!]
% \centering
% \scriptsize
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & loss function & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{B}$ (24) & -- & $30.59 \pm 5.40$& $29.55 \pm 2.77$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{B}$ (24) & BCE binary masks, sigmoid & $31.52 \pm 6.00$ & $30.63 \pm 3.81$ \\
%     Multi-Task UNet & $\mathcal{B}$ (24) + $\mathcal{U}$ & BCE binary masks/predictions, sigmoid & $33.03 \pm 7.25$ & $32.18 \pm 3.25$ \\
%     Multi-Task UNet & $\mathcal{B}$ (24) + $\mathcal{I}$ & BCE binary masks/predictions, $\mathcal{I}$-constrained, sigmoid & $34.55 \pm 5.20$ & $33.46 \pm 2.63$ \\
%     Multi-Task UNet & $\mathcal{B}$ (24) + $\mathcal{I}$ & BCE binary masks/predictions, $\mathcal{I}$-constrained, sigmoid, MIL & $-- \pm --$ & $-- \pm --$ \\
%     \hline    
%     \hline
%     UNet & $\mathcal{B}$ (\textbf{all}) & -- & $39.65 \pm 3.12$ & $38.45 \pm 4.44$ \\
%     Multi-Task UNet & $\mathcal{B}$ (\textbf{all}) & BCE binary masks & $39.71 \pm 2.81$ & $39.25 \pm 3.83$ \\
%     \hline
% \end{tabular}
% \caption{Ablation and comparison for using a L1-loss.}
% \label{fig:output_head}
% \end{table*}



% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|l|c|c|c|l|l|l|l}
%     & Supervision & batch size & infer. & loss function & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (24) & 16 & -- & -- & $46.84 \pm 6.49$& $48.63 \pm 5.17$ \\
%     \hdashline
%     M-T UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 16 & -- & binary masks/pred, $\mathcal{I}$-cons. & $57.24 \pm 5.74$ & $57.92 \pm 7.33$ \\
%     \red{X} M-T UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & stud & binary masks/pred, $\mathcal{I}$-cons., mean teacher & $58.26 \pm 4.27$ & $58.89 \pm 7.90$ \\
%     \red{X} M-T UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & stud & binary masks/pred, $\mathcal{I}$-cons., mean teacher + aug & $\textbf{58.54} \pm \textbf{3.62}$ & $\textbf{59.06} \pm \textbf{8.07}$ \\
%     \red{X} M-T UNet \red{R} & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & teach & binary masks/pred, $\mathcal{I}$-cons., mean teacher & $-- \pm --$ & $-- \pm --$ \\
%     \red{X} M-T UNet \red{R} & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & teach & binary masks/pred, $\mathcal{I}$-cons., mean teacher + aug & $-- \pm --$ & $-- \pm --$ \\
%     M-T UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & -- & binary masks/pred, $\mathcal{I}$-cons. & $57.18 \pm 6.37$ & $57.50 \pm 7.89$ \\
%     M-T UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & 10 & -- & binary masks/pred, $\mathcal{I}$-cons. + aug & $58.32 \pm 3.63$ & $58.03 \pm 6.85$ \\
%     \hline    
%     \hline
%     UNet & $\mathcal{M}$ (\textbf{all}) & 16 & -- & -- & $62.42 \pm 4.11$ & $62.09 \pm 4.77$\\
%     \red{X} M-T UNet & $\mathcal{M}$ (\textbf{all}) & 10 & stud & binary masks/pred, $\mathcal{I}$-cons., mean teacher & $65.66 \pm 3.57$ & $67.07 \pm 4.09$ \\
%     \red{X} M-T UNet & $\mathcal{M}$ (\textbf{all}) & 10 & stud & binary masks/pred, $\mathcal{I}$-cons., mean teacher + aug & $66.83 \pm 3.37$ & $66.79 \pm 4.96$ \\
%     \hline
% \end{tabular}
% \caption{Ablation for mean teacher.}
% \label{fig:mean_teacher_ablation}
% \end{table*}



% \begin{table*}[h!]
% \centering
% \scriptsize
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & loss function & mIoU val & mIoU test \\
%     \hline
%     UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & -- & $44.07 \pm 7.98$ & $45.48 \pm 6.83$ \\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & BCE binary masks, sigmoid & $47.53 \pm 8.56$ & $48.32 \pm 7.28$ \\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & BCE binary bb/masks/predictions, sigmoid & $39.59 \pm 9.38$ & $44.95 \pm 7.90$ \\
%     Multi-Task UNet (200 epochs) & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & BCE binary bb/masks/predictions, sigmoid & $45.33 \pm 10.86$ & $47.84 \pm 6.26$ \\
%     Multi-Task UNet (1000 epochs) & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & BCE binary bb/masks/predictions, sigmoid & $44.69 \pm 10.12$ & $45.73 \pm 9.39$ \\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & BCE binary bb/masks/predictions(mask only), sigmoid & $43.60 \pm 9.58$ & $47.31 \pm 4.38$ \\
%     Multi-Task UNet (200 epochs) & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & BCE binary bb/masks/predictions(mask only), sigmoid & $46.21 \pm 8.45$ & $48.64 \pm 8.17$ \\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{I}$ & BCE binary bb/masks/predictions, $\mathcal{I}$-constrained, sigmoid & $-- \pm --$ & $-- \pm --$ \\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{I}$ & BCE binary masks/predictions, $\mathcal{B}$- and $\mathcal{I}$-constrained, sigmoid, no $\mathcal{B}$-CE loss & $-- \pm --$ & $-- \pm --$ \\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{I}$ & BCE binary bb/masks/predictions, $\mathcal{I}$-constrained, sigmoid, MIL & $-- \pm --$ & $-- \pm --$ \\
%     \hline    
%     \hline
%     UNet & $\mathcal{B}$ (\textbf{all}) & -- & $39.65 \pm 3.12$ & $38.45 \pm 4.44$ \\
%     Multi-Task UNet & $\mathcal{B}$ (\textbf{all}) & BCE binary masks & $39.71 \pm 2.81$ & $39.25 \pm 3.83$ \\
%     \hdashline
%     UNet & $\mathcal{M}$ (\textbf{all}) & -- & $62.42 \pm 4.11$ & $62.09 \pm 4.77$\\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) & BCE binary masks & $65.39 \pm 3.89$ & $66.66 \pm 3.98$ \\
%     \hline
% \end{tabular}
% \caption{Ablation and comparison for using a L1-loss.}
% \label{fig:output_head}
% \end{table*}


% \begin{table*}[h!]
% \begin{tabular}{r|l|c|l|l|l|l}
%     & Supervision & \#clusters& IRF & SRF & PED & mIoU \\
%     \hline
%     UNet (100 epochs) & $\mathcal{M}$ (\textbf{all}) & -- & $ 57.92 \pm 6.22$ & $78.13 \pm 10.28$ & $53.25 \pm 11.80$ & $63.10 \pm 3.79$\\
%     UNet (200 epochs) & $\mathcal{M}$ (\textbf{all}) & -- & $57.54 \pm 5.71$ & $76.70 \pm 13.58$ & $52.95 \pm 9.44$ & $62.39 \pm 4.51$\\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 10 & $58.73 \pm 5.77$ & $80.13 \pm 8.58$ & $56.16 \pm 9.01$ & $\textbf{65.01} \pm \textbf{2.75}$\\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 20 & $58.27 \pm 5.47$ & $79.58 \pm 9.07$ & $56.52 \pm 9.67$ & $64.79 \pm 3.87$\\
%     Multi-Task UNet & $\mathcal{M}$ (\textbf{all}) + $\mathcal{U}$ & 40 & $57.27 \pm 6.68$ & $80.17 \pm 8.45$ & $57.42 \pm 8.62$ & $64.95 \pm 3.45$\\
%     \hline
% \end{tabular}
% \caption{Ablation for the number of heads for iic loss on the validation set of the Spectralis vendor.}
% \end{table*}

% \clearpage

% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|l|l|l|l|l}
%     & Supervision & IRF & SRF & PED & mIoU \\
%     \hline
%     UNet & $\mathcal{M}$ (\textbf{all}) & $ 57.92 \pm 6.22$ & $78.13 \pm 10.28$ & $53.25 \pm 11.80$ & $63.10 \pm 3.79$\\
%     \hline
%     UNet & $\mathcal{M}$ (3) & $ 19.57 \pm 12.47$ & $14.99 \pm 17.15$ & $6.72 \pm 7.95$ & $13.76 \pm 6.69$\\
%     Multi-Task UNet & $\mathcal{M}$ (3) + $\mathcal{U}$ & $17.89 \pm 14.31$ & $25.62 \pm 22.32$ & $14.03 \pm 12.27$ & $19.18 \pm 7.42$\\
%     Multi-Task UNet & $\mathcal{M}$ (3) + $\mathcal{I}$ & $ 16.95 \pm 16.22$ & $24.39 \pm 19.06$ & $8.09 \pm 11.22$ & $16.48 \pm 9.07$\\
%     \hdashline
%     UNet & $\mathcal{M}$ (6) & $ 26.50 \pm 11.50$ & $30.76 \pm 16.75$ & $16.70 \pm 9.74$ & $24.65 \pm 8.61$\\
%     Multi-Task UNet & $\mathcal{M}$ (6) + $\mathcal{U}$ & $25.28 \pm 15.98$ & $38.61 \pm 18.55$ & $23.89 \pm 11.85$ & $29.26 \pm 12.16$\\
%     Multi-Task UNet & $\mathcal{M}$ (6) + $\mathcal{I}$ & $ 27.20 \pm 16.25$ & $47.25 \pm 19.56$ & $20.88 \pm 11.83$ & $31.78 \pm 10.25$\\
%     \hdashline
%     UNet & $\mathcal{M}$ (12) & $37.20 \pm 9.08$ & $42.28 \pm 23.42$ & $22.07 \pm 11.33$ & $33.85 \pm 8.88$\\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{U}$ & $39.62 \pm 12.78$ & $55.36 \pm 17.85$ & $25.13 \pm 15.47$ & $40.04 \pm 8.40$\\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{I}$ & $ 40.55 \pm 12.15$ & $60.22 \pm 16.61$ & $23.39 \pm 17.27$ & $41.38 \pm 7.35$\\
%     \hdashline
%     UNet & $\mathcal{M}$ (24) & $ 46.15 \pm 8.80$ & $61.27 \pm 21.44$ & $35.32 \pm 13.21$ & $47.58 \pm 6.48$\\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{U}$ & $46.91 \pm 7.52$ & $70.81 \pm 16.10$ & $39.55 \pm 13.22$ & $52.42 \pm 5.28$\\
%     Multi-Task UNet & $\mathcal{M}$ (24) + $\mathcal{I}$ & $ 50.64 \pm 8.38$ & $71.69 \pm 13.40$ & $40.42 \pm 15.00$ & $54.25 \pm 4.18$\\
%     \gray{Multi-Task UNet} & $\mathcal{M}$ (24) + $\mathcal{SL}$ & $50.54 \pm 8.81$ & $69.06 \pm 19.19$ & $39.76 \pm 12.02$ & $53.12 \pm 5.60$\\
%     \hline
%     \hline
%     UNet & $\mathcal{B}$ (\textbf{all}) & $22.09 \pm 5.26$ & $51.77 \pm 9.41$ & $39.45 \pm 6.41$ & $37.77 \pm 2.71$ \\
%     \hline
%     UNet & $\mathcal{B}$ (3) & $ 12.98 \pm 4.44$ & $15.23 \pm 11.32$ & $5.50 \pm 4.81$ & $11.24 \pm 5.33$\\
%     Multi-Task UNet & $\mathcal{B}$ (3) + $\mathcal{U}$ & $12.97 \pm 4.78$ & $24.78 \pm 19.35$ & $7.11 \pm 8.59$ & $14.95 \pm 7.78$\\
%     Multi-Task UNet & $\mathcal{B}$ (3) + $\mathcal{I}$ & $ 12.89 \pm 5.39$ & $29.54 \pm 19.10$ & $7.54 \pm 8.43$ & $16.66 \pm 7.90$\\
%     \hdashline
%     UNet & $\mathcal{B}$ (6) & $ 15.56 \pm 6.03$ & $17.90 \pm 16.31$ & $15.76 \pm 10.18$ & $16.41 \pm 7.84$\\
%     Multi-Task UNet & $\mathcal{B}$ (6) + $\mathcal{U}$ & $17.31 \pm 6.10$ & $24.07 \pm 18.50$ & $12.43 \pm 9.32$ & $17.93 \pm 8.66$\\
%     Multi-Task UNet & $\mathcal{B}$ (6) + $\mathcal{I}$ & $ 17.77 \pm 8.42$ & $33.13 \pm 11.97$ & $12.83 \pm 10.11$ & $21.25 \pm 7.08$\\
%     \hdashline
%     UNet & $\mathcal{B}$ (12) & $ 18.20 \pm 4.59$ & $32.45 \pm 20.39$ & $20.78 \pm 11.70$ & $23.81 \pm 8.42$\\
%     Multi-Task UNet & $\mathcal{B}$ (12) + $\mathcal{U}$ & $19.49 \pm 5.82$ & $37.47 \pm 18.63$ & $24.12 \pm 10.16$ & $27.03 \pm 7.26$\\
%     Multi-Task UNet & $\mathcal{B}$ (12) + $\mathcal{I}$ & $19.23 \pm 6.33$ & $38.29 \pm 11.34$ & $18.58 \pm 11.00$ & $25.37 \pm 5.58$\\
%     \hdashline
%     UNet & $\mathcal{B}$ (24) & $ 20.22 \pm 3.64$ & $44.79 \pm 14.74$ & $27.40 \pm 11.75$ & $30.81 \pm 6.63$\\
%     Multi-Task UNet & $\mathcal{B}$ (24) + $\mathcal{U}$ & $20.79 \pm 4.60$ & $47.83 \pm 15.53$ & $32.57 \pm 13.86$ & $33.73 \pm 7.34$\\
%     Multi-Task UNet & $\mathcal{B}$ (24) + $\mathcal{I}$ & $20.49 \pm 3.92$ & $48.79 \pm 9.34$ & $26.97 \pm 9.74$ & $32.08 \pm 5.53$\\
%     \hline
%     \hline
%     UNet & $\mathcal{I}$ (\textbf{all}) & $4.29 \pm 3.21$ & $10.00 \pm 6.25$ & $4.13 \pm 2.71$ & $6.14 \pm 1.74$\\
%     \hline
%     \hline
%     Multi-Task UNet & $\mathcal{M}$ (3) + $\mathcal{B}$ (3) & $16.10 \pm 11.72$ & $12.22 \pm 13.25 $ & $8.55 \pm 8.26$ & $12.29 \pm 7.34$\\
%     Multi-Task UNet & $\mathcal{M}$ (3) + $\mathcal{B}$ (3) + $\mathcal{U}$ & $14.94 \pm 12.58$ & $22.93 \pm 22.77$ & $12.85 \pm 14.14$ & $16.91 \pm 11.34$\\
%     Multi-Task UNet & $\mathcal{M}$ (3) + $\mathcal{B}$ (3) + $\mathcal{I}$ & $19.79 \pm 14.73 $ & $35.09 \pm 24.14 $ & $6.14 \pm 5.92$ & $20.34 \pm 6.45$\\
%     %\blue{Multi-Task UNet} & $\mathcal{M}$ (3) + $\mathcal{B}$ (3) + $\mathcal{I}$ \red{running}& $-- \pm --$ & $-- \pm -- $ & $-- \pm --$ & $-- \pm --$\\
%     \hdashline
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & $40.77 \pm 8.29$ & $60.88 \pm 18.90$ & $32.36 \pm 15.91$ & $44.67 \pm 8.00$\\
%     %\blue{Multi-Task UNet} & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) \red{running} & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ & $-- \pm --$\\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & $38.66 \pm 12.58$ & $61.43 \pm 18.46$ & $35.60 \pm 15.08$ & $45.23 \pm 8.29$\\
%     %\blue{Multi-Task UNet} & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{U}$ & $40.69 \pm 9.60$ & $65.31 \pm 15.67$ & $32.90 \pm 14.47$ & $46.30 \pm 7.05$\\
%     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{I}$ & $40.73 \pm 9.42$ & $63.89 \pm 14.02 $ & $34.29 \pm 12.71$ & $46.30 \pm 6.92$\\
%     %\blue{Multi-Task UNet} & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) + $\mathcal{I}$ \red{running} & $-- \pm --$ & $-- \pm -- $ & $-- \pm --$ & $-- \pm --$\\
%     \hline
% \end{tabular}
% \caption{Validation results across 10 splits, for the Spectralis vendor, IoU (without background) $\pm$ standard deviation. The abbreviations $\mathcal{M}$, $\mathcal{B}$, $\mathcal{I}$ stand for Mask-, Bounding Box- and Image-level supervision signals, the numbers in brackets show how many examples with this kind of supervision were used to train the models. \red{3x for each vendor}}
% \end{table*}


% % \begin{table*}[h!]
% % \begin{tabular}{r|l|c|l|l|l|l}
% %     & Supervision & Loss & IRF & SRF & PED & mIoU \\
% %     \hline
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{CE}$ & $40.77 \pm 8.29$ & $60.88 \pm 18.90$ & $32.36 \pm 15.91$ & $44.67 \pm 8.00$\\
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{MIL}$ & $37.09 \pm 7.82$ & $52.14 \pm 25.09$ & $27.48 \pm 14.37$ & $38.94 \pm 10.25$\\
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{MIL}, BB_{bkg}^1$ & $38.75 \pm 10.52$ & $53.23 \pm 23.17$ & $25.23 \pm 14.33$ & $39.07 \pm 8.62$\\
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{MIL}, BB_{bkg}^2$ & $38.21 \pm 9.68$ & $53.16 \pm 19.79$ & $25.39 \pm 15.23$ & $38.92 \pm 9.71$\\
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{MIL}, BB_{bkg}^{1,2}$ & $36.86 \pm 10.86$ & $52.90 \pm 22.61$ & $25.91 \pm 13.54$ & $38.56 \pm 10.14$\\
% %     Multi-Task UNet & $\mathcal{M}$ (12) + $\mathcal{B}$ (12) & \tiny$Mask_{CE}, BB_{CE}, BB_{bkg}^{2}$ & $-- \pm --$ & $-- \pm --$ & $-- \pm --$ & $-- \pm --$\\
% %     \hline
% % \end{tabular}
% % \caption{Ablation for how to combine Mask- and Bounding Box-based losses on the validation set of the Spectralis vendor. The losses are: $Mask_{CE}, BB_{CE}, BB_{MIL}, BB_{bkg}^1, BB_{bkg}^2$ standing for standard cross-entropy loss using pixel-wise masks, cross-entropy loss using bounding boxes as 'noisy pixel-wise masks', a MIL-based loss for bounding boxes, a cross-entropy loss for the background-class in bounding box annotations used on (1) the bounding box-based output-head and (2) the mask-based output-head.}
% % \end{table*}

% \begin{table*}[h!]
% \centering
% \begin{tabular}{r|l|l|l}
%     & Supervision & mIoU val & mIoU test\\
%     \hline 
%     UNet&$\mathcal{I}$&$ 5.49 \pm 1.82 $&$ 5.25 \pm 2.02 $\\ 
%     \hline 
%     UNet&$\mathcal{M}(3) $&$ 14.00 \pm 7.24 $&$ 15.48 \pm 6.00 $\\ 
%     Multi-Task UNet&$\mathcal{M}(3) $ + $\mathcal{I}$&$ 13.91 \pm 5.67 $&$ 12.95 \pm 6.07 $\\ 
%     Multi-Task UNet&$\mathcal{M}(3) $ + $\mathcal{U}$&$ 20.02 \pm 7.19 $&$ 19.53 \pm 6.71 $\\ 
%     \hdashline
%     UNet&$\mathcal{M}(6) $&$ 23.68 \pm 8.49 $&$ 26.58 \pm 8.00 $\\ 
%     Multi-Task UNet&$\mathcal{M}(6) $ + $\mathcal{I}$&$ 29.00 \pm 10.61 $&$ 27.69 \pm 8.72 $\\ 
%     Multi-Task UNet&$\mathcal{M}(6) $ + $\mathcal{U}$&$ 29.09 \pm 11.43 $&$ 30.55 \pm 6.96 $\\ 
%     \hdashline
%     UNet&$\mathcal{M}(12) $&$ 33.83 \pm 7.16 $&$ 35.72 \pm 6.56 $\\ 
%     Multi-Task UNet&$\mathcal{M}(12) $ + $\mathcal{I}$&$ 40.04 \pm 10.91 $&$ 38.97 \pm 7.60 $\\ 
%     Multi-Task UNet&$\mathcal{M}(12) $ + $\mathcal{U}$&$ 39.23 \pm 10.06 $&$ 40.52 \pm 7.41 $\\ 
%     \hdashline
%     UNet&$\mathcal{M}(24) $&$ 45.91 \pm 5.83 $&$ 46.75 \pm 5.79 $\\ 
%     Multi-Task UNet&$\mathcal{M}(24) $ + $\mathcal{I}$&$ 52.02 \pm 4.52 $&$ 49.73 \pm 6.18 $\\ 
%     Multi-Task UNet&$\mathcal{M}(24) $ + $\mathcal{U}$&$ 51.89 \pm 6.52 $&$ 51.16 \pm 7.77 $\\ 
%     \hline
%     Multi-Task UNet&$\mathcal{B}(3) $&$ 11.92 \pm 4.64 $&$ 12.19 \pm 3.66 $\\ 
%     Multi-Task UNet&$\mathcal{B}(3) $ + $\mathcal{I}$&$ 13.77 \pm 5.82 $&$ 11.22 \pm 6.61 $\\ 
%     Multi-Task UNet&$\mathcal{B}(3) $ + $\mathcal{U}$&$ 14.81 \pm 6.02 $&$ 16.37 \pm 7.06 $\\ 
%     \hdashline
%     Multi-Task UNet&$\mathcal{B}(6) $&$ 15.46 \pm 6.45 $&$ 15.97 \pm 4.52 $\\ 
%     Multi-Task UNet&$\mathcal{B}(6) $ + $\mathcal{I}$&$ 20.55 \pm 4.66 $&$ 17.82 \pm 7.62 $\\
%     Multi-Task UNet&$\mathcal{B}(6) $ + $\mathcal{U}$&$ 18.77 \pm 8.48 $&$ 18.81 \pm 8.48 $\\
%     \hdashline 
%     UNet&$\mathcal{B}(12) $&$ 22.26 \pm 7.42 $&$ 24.83 \pm 3.77 $\\ 
%     Multi-Task UNet&$\mathcal{B}(12) $ + $\mathcal{I}$&$ 25.39 \pm 5.18 $&$ 24.19 \pm 4.28 $\\ 
%     Multi-Task UNet&$\mathcal{B}(12) $ + $\mathcal{U}$&$ 26.90 \pm 5.77 $&$ 27.10 \pm 4.35 $\\ 
%     \hdashline
%     \red{missing}& -- &$-- \pm --$&$-- \pm --$\\ 
%     \red{missing}& -- &$-- \pm --$&$-- \pm --$\\ 
%     Multi-Task UNet&$\mathcal{B}(24) $ + $\mathcal{I}$&$ 33.74 \pm 5.60 $&$ 31.52 \pm 3.54 $\\ 
%     \hline
%     Multi-Task UNet&$\mathcal{M}(3) $ + $\mathcal{B}(3) $&$ 14.50 \pm 9.39 $&$ 16.31 \pm 10.46 $\\ 
%     Multi-Task UNet&$\mathcal{M}(3) $ + $\mathcal{B}(3) $ + $\mathcal{I}$&$ 18.43 \pm 7.21 $&$ 16.87 \pm 9.66 $\\ 
%     \red{missing}& -- &$-- \pm --$&$-- \pm --$\\ 
%     \hdashline
%     \red{missing}& -- &$-- \pm --$&$-- \pm --$\\
%     Multi-Task UNet&$\mathcal{M}(12) $ + $\mathcal{B}(12) $ + $\mathcal{I}$&$ 45.65 \pm 7.23 $&$ 46.11 \pm 6.49 $\\ 
%     \red{missing}& -- &$-- \pm --$&$-- \pm --$\\
%     \hline
% \end{tabular}
% \end{table*}

% \clearpage
